Mechanics of Next Token Prediction with Self-Attention

Transformer-based language models are trained on large datasets to predict the next token given an input sequence. Despite this simple training objective, they have led to revolutionary advances in natural language processing. Underlying this success is the self-attention mechanism. In this work, we ask: $\textit{What}$ $\textit{does}$ $\textit{a}$ $\textit{single}$ $\textit{self-attention}$ $\textit{layer}$ $\textit{learn}$ $\textit{from}$ $\textit{next-token}$ $\textit{prediction?}$ We show that training self-attention with gradient descent learns an automaton which generates the next token in two distinct steps: $\textbf{(1)}$ $\textbf{Hard}$ $\textbf{retrieval:}$ Given input sequence, self-attention precisely selects the $\textit{high-priority}$ $\textit{input}$ $\textit{tokens}$ associated with the last input token. $\textbf{(2)}$ $\textbf{Soft}$ $\textbf{composition:}$ It then creates a convex combination of the high-priority tokens from which the next token can be sampled. Under suitable conditions, we rigorously characterize these mechanics through a directed graph over tokens extracted from the training data. We prove that gradient descent implicitly discovers the strongly-connected components (SCC) of this graph and self-attention learns to retrieve the tokens that belong to the highest-priority SCC available in the context window. Our theory relies on decomposing the model weights into a directional component and a finite component that correspond to hard retrieval and soft composition steps respectively. This also formalizes a related implicit bias formula conjectured in [Tarzanagh et al. 2023]. We hope that these findings shed light on how self-attention processes sequential data and pave the path toward demystifying more complex architectures.

==> sec/gd_backup_.tex <==
\section{Implicit Bias of Self-Attention}
To proceed, we wish to identify the Implicit bias of self-attention on general next-token prediction problems. This necessitates the general form \eqref{graph svm} as well as additional ideas. To start, we make the following simplifying assumption on the tokens.
% \begin{assumption}[Orthogonal token embeddings]\label{assume orth}  Embeddings satisfy $\Eb\Eb^\top=\Iden_K$.
% \end{assumption}
% \begin{assumption} [Assumptions on SCCs] \label{assume scc}    Given $\data$, assume that there exists $k \in [K]$, there are at least two SCCs in $\Gck$, i.e., $N_k \geq 2$. \yl{[Lizzie: How about assuming $\Wm\neq0$? This assumption might not be enough.]}
% \redp{Shaw: Lemma 6 builds the equivalence of Assumption 6 and $\Wm \neq 0$.}
% \end{assumption}
% \redp{We need this assumption such that there is at least one directed edge between nodes in different SCCs.}\\
% The next theorem states the directional bias of self-attention on general data to the solution of \eqref{graph svm}.
% \begin{theorem}\label{thm graph bias} Suppose Assumptions \ref{assume iden}\&\ref{assume loss} hold. Consider the GD iterations $\W_{k+1}=\W_k-\frac{1}{L}\nabla\Lc(\W_k)$ where $L$ is the smoothness of $\Lc(\W)$. Suppose \eqref{graph svm} is feasible and $\Wm$ denotes its solution. Starting from any $\W_0$, we have
% \begin{align}
% \lim_{k\rightarrow\infty}\frac{\W_k}{\tf{\W_k}}=\frac{\Wm}{\tf{\Wm}}
% \end{align}
% Additionally, regularization path $\bar{\W}_R=\arg\min_{\tf{\W}\leq R}\Lc(\W)$ obeys the same limit.\redp{simpler to prove}
% \end{theorem}
% \redp{If we can't prove above (for whatever reason), we can still convert it to a less formal discussion. I think we can though}

% While Theorem \ref{thm graph bias} provides the directional bias of self-attention, as we shall see, it does not truly capture the essence of its solution. To this end, we will introduce the so-called finite-correction term first proposed in \cite{}. We remark that \cite{}'s proposal is highly informal and is developed for understanding the MLP layer following self-attention. In contrast, we will develop clear formulas and theory that shed light on the mechanics of next-token prediction. Our theory relies on the strongly-connected components (SCC) of the next-token graph.

% \begin{definition} [Finite correction $\Wf$] \label{def finite correct} $\Wf$ is obtained as the min norm solution of the empirical risk minimization over the cyclic subset $\bdata$ per Definition \ref{cyc sub}. Concretely, $\Wf=\arg\min_{\W\in\Wcf}\tf{\W}$ where $\Wcf$ denotes the set of ERM solutions over $\bdata$ i.e.
% \begin{align}\label{wfin soln}
% %\Lc_{\texttt{cyc}}(\W):=
% \Wcf=\arg\min_{\W}\frac{1}{|\bdata|}\sum_{(\X,y)\in\bdata} \ell(\cb_{y}^\top\X^\top \sft{\X\W\xl}).
% \end{align}

% We also define the subspace $\Scf\in\R^{d\times d}$ associated to $\Wf$ as follows. For each non-singleton SCC $\Cck_i$, define its mean embedding $\bmu^{(k)}_i=\frac{1}{|\Cck_i|}\sum_{j\in \Cck_i} \eb_j$. Let $\Scf$ be the span of all matrices $(\eb_j-\bmu^{(k)}_i)\eb_k^\top$ for $j\in\Cck_i,i\in[N_k],k\in[K]$.
% %For each last token $\xl=\eb_k$ and SCC $\Cck$
% %and let $\Lc_\st=\arg\min_{\W}\Lc_{\texttt{cyc}}(\W)$. 

% \end{definition}
We have the following results regarding finite correction $\Wf$ and SVM-induced direction $\Wm$. \redp{I am stating these in theorem/lemma form to make the claims formal (although we don't have proofs yet).}
\begin{lemma}\label{lemma ortho} Suppose Assumption \ref{assume orth} holds and consider Definition \ref{def finite correct}. We have that $\Wf\subset \Scf$ and $\Wm\perp \Scf$. Thus, $\Wf$ and $\Wm$ are orthogonal i.e.~$\li\Wf,\Wm\ri=0$.
\end{lemma}
\redp{Proof strategy: $\Scf$ can be decomposed into orthogonal subspaces based on $k\in[K]$ and individual SCCs within fixed $k$. Subtracting mean embedding $\bmu$ does not change softmax output over $\Wf$ but makes $\Wf$ orthogonal to $\Wm$ as $\Wm$ can only have $\bmu$ direction.}


\begin{theorem}\label{thm: decompose} 
Consider the setting of Theorem \ref{thm graph bias} and suppose Assumption \ref{assume orth} holds as well. From zero initialization, gradient descent iterates obey \redp{alternatively, we can state the theorem for regularization path}
\begin{align}
\lim_{k\rightarrow\infty}\frac{\prj_{\Scp}(\W_k)}{\tf{\prj_{\Scp}(\W_k)}}= \frac{\Wm}{\tf{\Wm}}\quad\text{AND}\quad\lim_{k\rightarrow\infty}\prj_{\Scf}(\W_k)= \Wf.
\end{align}
Above $\prj$ denotes the subspace projection with respect to Euclidean distance.

\end{theorem}
Together, the limits above imply the decomposition $\W_k\approx C_k\cdot\Wm+\Wf$ for an appropriate $C_k>0$.
\redp{What loss functions will give the finite solution.}
\textbf{Understanding training risk of GD iterations.} \redp{As $k\rightarrow\infty$ and assuming realizability: (1) Over $\data-\cdata$, self-attention should precisely output the correct label embedding i.e.~$\eb_y$. On the other hand, over the cyclic subset $\cdata$, the probabilities will be split and self-attention will output a convex combination of input tokens within the same SCC as $y$.}

==> sec/next_token.tex <==
\section{Next-token prediction}
\subsection{Preliminaries}
\begin{definition} For a input $\X_i$, each token $\x_{it}$ is drawn independently from a vocabulary $\Z = \{\z_k\}_{k = 1}^K \in \R^{K \times d}$. The label of each token $z_{\alpha_k}$ is also drawn from $\Z$. The task is to predict the next token of the input sequence, which is the label of the last token $x_{T_i} = \z_{k_i}$ is $\y_i = z_{\bal_{k_i}}$
\end{definition}
Consider a single-layer self-attention problem that predicts the next token using the input with $T$ tokens. 
\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=green!1!white]
\vspace{5pt}
\begin{equation}\tag{Att-SVM}
% \Wm_\ell=\arg\min_{\W}\tf{\W}
% \quad \text{subj. to} \quad (\x_{i\op_i}-\x_{it})^\top\W((2^{\ell-1}-1)\x_{i\op_i}+\x_{it})\geq 1\quad  \text{for all} \quad t \neq \op_i,~i\in[n],~\ell\in[L].
\Wm = \arg\min_{\W} \tf{\W} \quad \text{subj. to} \quad (\z_{\bal_{k_i}} - \z_{j} )^\top\W \z_{k_i} \geq 1 \quad \text{for all} \quad j \neq \bal_{k_i},~i\in[n]
\label{eqn:sattnsvm}
\end{equation}
\end{tcolorbox}

\textbf{SVM problem for non-separable case. }Where input sequences with the same last token $x_T$ may correspond to multiple tokens, $g: x_T \to \{z_t | t \in \mathcal{O} \}$, suppose $m_t = p(z_{\alpha_k} =z_{t} | x_T)$. Following \cite{tarzanagh2023transformers}, we decompose $\W(k)$ into two components
\begin{equation}
    \W(k) \approx \W^{fin} + \tf{\W(k)}\cdot \bar{\W}^{mm}
\end{equation}
where $\W^{fin}$ is the finite component to assign non-zero softmax probabilities and $\bar{\W}^{mm}$ is the directional component with $\tf{\bar{\W}^{mm}}$ = 1.
\begin{itemize}
    \item Finite component: Intuitively, the finite component should assign softmax probabilities according to the conditional probabilities $m_t$ given $x_T$ to achieve the optimal loss. This is given by: 
    \begin{equation}
        (\z_{t} - \z_{\tau})^\top\W^{fin} x_T = \log \frac{m_t}{m_\tau}, \quad \text{for all} \quad t, \tau \in \mathcal{O}_i, i \in [n].
    \end{equation}
    \item Directional component: $\bar{\W}^{mm}$ helps to select the tokens in $\mathcal{O}$ and suppress the other tokens in $\bar{\mathcal{O}} = [K] - \mathcal{O}$ by setting the softmax probabilities as 0. There are two constraints that $\W^{mm}$ should satisfy as below: 
\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=green!1!white]
\vspace{5pt}
\begin{equation}\tag{Gen-SVM}
% \Wm_\ell=\arg\min_{\W}\tf{\W}
% \quad \text{subj. to} \quad (\x_{i\op_i}-\x_{it})^\top\W((2^{\ell-1}-1)\x_{i\op_i}+\x_{it})\geq 1\quad  \text{for all} \quad t \neq \op_i,~i\in[n],~\ell\in[L].
\Wm = \arg\min_{\W} \tf{\W} \quad \text{subj. to} 
    \begin{cases} 
    (\z_{t} - \z_{\tau})^\top\W \z_{k_i} = 0, & \text{for all} \quad t, \tau \in \mathcal{O}_i \\ 
    (\z_{t} - \z_{\tau} )^\top\W \z_{k_i} \geq 1, & \text{for all} \quad t \in \mathcal{O}_i, \tau \in \bar{\mathcal{O}}_i \\ 
    \end{cases}  ~ i\in[n]
\label{eqn:rattnsvm}
\end{equation}
\end{tcolorbox}
\end{itemize}


% \begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=green!1!white]
% \vspace{5pt}
\begin{assumption} \label{assump:loss}
Over any bounded interval: (i) $\ell : \R \to \R$ is strictly decreasing and bounded from below; (ii) The derivative of $\ell$, denoted as $\ell'$, is $M_0$-Lipschitz continuous; and (iii) $|\ell'(u)| \leq M_1$
\end{assumption}
% In our analysis, we used the correlation loss $\ell(u) = -u$  


\begin{tcolorbox}[colback=white!5!white,colframe=black!5!black,colback=green!1!white]
\textbf{Problem definition. } 
\begin{equation}\tag{W-ERM}
    \mathcal{L}(\W) = \frac{1}{n}\sum_{i=1}^n \ell \left(\y_i^\top \X_i^\top \sft{\X_i\W \x_{T_i}}\right)
\label{eq:werm}
\end{equation}
% Suppose $Y_i = \alpha_{ki} \in [K], s_{Yi} =  $
% \begin{equation}\tag{CE loss}
%     \mathcal{L}(\W) = \frac{1}{n}\sum_{i=1}^n -\log s_{Y_i}^i = \frac{1}{n}\sum_{i=1}^n -\log \left( \frac{e^{z_{iY_i}^{\top}Wx_{T_i}}}{\sum_{t=1}^T e^{\x_{it}^{\top}W\x_{T_i}}}\right)
% \label{eq:werm}
% \end{equation}
\textbf{Optimization Process. } Given $\W(0) \in \R^{d \times d}, \eta > 0, \text{ for } k \geq 0 \text{ do:}$  
\begin{equation}\tag{W-GD} \label{eq:wgd}
    \W(k+1) = \W(k) - \eta \nabla \mathcal{L}(\W(k)) 
\end{equation}
\end{tcolorbox}

\begin{definition}[Token Score] Given a input $X_i$ and the label of the last token in the sequence $\y_i \in \R^{d}$, the token score of a token $x_{it}$ if input $\X_i$ is defined as $\gamma_{it} = \y_i^{\top}\x_{it}$. 
\end{definition}

\begin{lemma} \label{le:vloss}
    Under Assumption \ref{assump:loss}, $\nabla \mathcal{L}(\W)$ is $L_{\W}$-Lipschitz continuous ,where \textcolor{red}{$a_i = \|z_{\alpha_{k_i}}\|\|z_{k_i}\|^2\|\X_i\|^3, b_i = M_0\|z_{\alpha_{k_i}}\| \|\X_i\| + 3M_1$} for all $i \in [n]$
    \begin{equation} \label{eq:vlwconst}
        L_{\W} \coloneqq \frac{1}{n}\sum_{i=1}^n a_i b_i
    \end{equation}
\end{lemma}





\subsection{Global convergence on equi-correlated tokens}
\begin{assumption}[Assumptions on token scores] \label{assump:token} First assume that te input sequence $X_i$ contain \textcolor{red}{all tokens} in the vocabulary. Below are the possible assumptions for token scores:
    \begin{enumerate}[label={\textnormal{{\textbf{\theassumption.\arabic*}}}}, wide, labelwidth=!,itemindent=!, labelindent=1pt, ref={\theassumption.\arabic*}]
        \item \label{assump:tokenA} \textbf{orthonormal tokens} $\forall j,k \in [K], \|\z_j\| = \|\z_k \| = 1, \langle {\z_j, \z_k} \rangle = 
            \begin{cases}
                0, & j \neq k \\ 
                1, & j = k
            \end{cases}$
        \item \label{assump:tokenB} \textbf{Equi-correlated tokens} $\forall j,k \in [K], \|\z_j\| = \|\z_k \| = 1, \langle {\z_j, \z_k} \rangle = 
            \begin{cases}
                \rho, & j \neq k \\ 
                1, & j = k
            \end{cases}$, where $\rho \in (0,1)$
        \item \label{assump:tokenC} \textcolor{red}{\textbf{Equiangular Tight Frame}} $\forall j,k \in [K], \|\z_j\| = \|\z_k \| = 1, |\langle {\z_j, \z_k} \rangle| = 
            \begin{cases}
                \rho, & j \neq k \\ 
                1, & j = k
            \end{cases}$, where $\rho \in (0,1)$
        \item \label{assump:tokenD} \textbf{Random tokens} $\|\z_j\| = 1, \forall j \in [K]$
    \end{enumerate}
\end{assumption}
\begin{theorem} \label{thm:vw} Supposing Assumption \ref{assump:loss} and \ref{assump:token} hold. Then, 
    \begin{itemize}
        \item There is no $\W $ satisfying $\nabla \mathcal{L}(\W) = 0$
        \item Algorithm \ref{eq:wgd} with the step size $\eta \leq \mathcal{O}(1 / L_W)$ and any initialization satisfies $\lim_{k \to \infty} \tf{\nabla \mathcal{L}(W(k))} = 0$ and $\lim_{k \to \infty} \tf{W(k)} = \infty$
    \end{itemize}
\end{theorem}
\begin{theorem} \label{thm:vwbias}
    Suppose Assumption \ref{assump:loss} on loss function and \ref{assump:token} on tokens' scores hold. Then, Algorithm \ref{eq:wgd} with the step size $\eta \leq \mathcal{O}(1 / L_W)$ and any initialization satisfies $\lim_{k \to \infty} \frac{\W(k)}{\tf{\W(k)}} = \frac{\Wm}{\tf{\Wm}}$
\end{theorem}

\newpage
% \begin{figure}[!ht]
%   \caption{ Global convergence behaviour of GD when training attention weights $\W$ using orthonormal data: }
% \begin{subfigure}{.4\textwidth}
%     \centering
%   \includegraphics[width=\linewidth]{Figures/Next-Token prediction/Next_Token_Ortho_Corr.png}
%   \caption{Correlation between GD solution and solution of \eqref{eqn:sattnsvm}}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
%     \centering
%   \includegraphics[width=\linewidth]{Figures/Next-Token prediction/Next_Token_Ortho_Bar.png}
%   \caption{Frequency of global convergence}
% \end{subfigure}
% \end{figure}

% \begin{figure}[!ht]
%   \caption{ Global convergence behaviour of GD when training attention weights $\W$ using equi-correlated data: }
% \begin{subfigure}{.4\textwidth}
%     \centering
%   \includegraphics[width=\linewidth]{Figures/Next-Token prediction/Next_Token_Equi_Corr.png}
%   \caption{Correlation between GD solution and solution of \eqref{eqn:sattnsvm}}
% \end{subfigure}
% \begin{subfigure}{.5\textwidth}
%     \centering
%   \includegraphics[width=\linewidth]{Figures/Next-Token prediction/Next_Token_Equi_Bar.png}
%   \caption{Frequency of global convergence}
% \end{subfigure}
% \end{figure}


\begin{figure}[!ht]
  \caption{Convergence behaviour of GD when training attention weights $\W$ with $\data$ dataset ($n = 5, T = K = 5, d = 10$) using NLL loss}
\begin{subfigure}{.45\textwidth}
    \centering
  \includegraphics[width=\linewidth]{Figures/Next-Token prediction/nll_default_n5_t5_k5_pos.png}
  \caption{Correlation between GD solution and solution of \eqref{graph svm}}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
    \centering
  \includegraphics[width=\linewidth]{Figures/Next-Token prediction/nll_default_n5_t5_k5_neg.png}
  \caption{1 - Correlation between GD solution and solution of \eqref{graph svm}}
\end{subfigure}
\end{figure}

\begin{figure}[!ht]
  \caption{Convergence behaviour of GD when training attention weights $\W$ with $\data$ dataset ($n = 5, T = K = 5, d = 10$) using CE loss}
\begin{subfigure}{.45\textwidth}
    \centering
  \includegraphics[width=\linewidth]{Figures/Next-Token prediction/ce_default_n5_t5_k5_pos.png}
  \caption{Correlation between GD solution and solution of \eqref{graph svm}}
\end{subfigure}
\begin{subfigure}{.45\textwidth}
    \centering
  \includegraphics[width=\linewidth]{Figures/Next-Token prediction/ce_default_n5_t5_k5_neg.png}
  \caption{1 - Correlation between GD solution and solution of \eqref{graph svm}}
\end{subfigure}
\end{figure}



==> sec/setup_backup_.tex <==
% \section{Problem Setup: ERM Problem and Next-Token Graph}
\section{Problem Setup}
\noindent\textbf{Notation.} Let $[n]$ denote set $\{1\cdots n\}$. For a subspace $\Sc$, let $\Sc^\perp$ denotes the orthogonal subspace of $\Sc$ and $\prj_\Sc$ denote the subspace projection with respect to Euclidean distance.

\noindent\textbf{Next-token prediction problem.} Let $\Eb=\begin{bmatrix}\eb_1~\dots~\eb_K\end{bmatrix}^\top\in\R^{K\times d}$ be the set of $K$ $d$-dimensional token embeddings. The next-token prediction is a multi-class classification problem and the goal is predicting the ID $y\in[K]$ of the next token given input sequence $\X=[\x_1~\dots~\x_T]^\top\in\R^{T\times d}$, where $\x_t\in\Eb,t\in[T]$.

Suppose that we have a training dataset $\data=(\X_i,y_i)_{i=1}^n\subset \R^{T_i\times d}\times [K]$, where $n$ is the number of sequences and we allow the sequences to have different lengths $T_i$, $i\in[n]$. Throughout, we denote $x_{it}$ as the scalar token IDs of the input token $\x_{it}$.

% \red{Throughout, we will use boldface label $\y\in\R^d$ to denote the embedding corresponding to scalar $y$, that is, $\y=\eb_y$. Conversely, we denote $\Xs\in[K]^T$ as the scalar token IDs of the input sequence $\X$. Thus, in vector form training data is $(\X_i,\y_i)_{i=1}^n$ whereas in sequence form it is $(\Xs_i,y_i)_{i=1}^n$.}

\noindent \textbf{Self-attention model.} We first consider a self-attention model when making a prediction on an input sequence $\X\in\R^{T\times d}$. Let $\xl:=\x_T$ being the last token of $\X$. To learn from $\X$, following the previous work \cite{tarzanagh2023transformers}, we denote the combined key-query weights by the trainable $\W\in\R^{d\times d}$ matrix, and assume identity value matrix. Then, self-attention outputs a token by composing the tokens of $\X$ as follows
\[ 
f_{\W}(\X)=\X^\top \sft{\X\W\xl}.
\]
Above $\sft{\cdot}$ is the softmax nonlinearity which weights tokens of $\X$ based on data-dependent probabilities $\sft{\X\W\xl}$, and $f_{\W}(\X)\in\R^d$ outputs composed token weighted by the probabilities.

\noindent \textbf{ERM problem.} Let $\Cb\in\R^{K\times d}$ be the linear classifier that reads the output token of self-attention and outputs per-class predictions $\hat{\y}\in\R^K$. Additionally, let $\ell(y,\hat{\y})$ be the loss function that assesses the mismatch between predictions $\hat{\y}$ and true label $y\in[K]$. Given training dataset $\data$, we consider the following empirical risk minimization problem
\begin{align}
\Lc(\Cb,\W)=\frac{1}{n}\sum_{i=1}^n \ell(y_i,\Cb\X_i^\top \sft{\X_i\W\xl_i}).\label{erm}
\end{align}
Throughout, we fix the linear head $\Cb$ and assume $\tf{\Cb}<\infty$. Let $\Lc(\W):=\Lc(\Cb,\W)$.  Although the head is fixed and linear, the problem is non-convex and non-linear due to the softmax operator. Therefore, in this work, we focus on optimizing attention weights $\W$ and build an SVM equivalence of it.

\subsection{Next-token Graph (NTG) of the Dataset}
Different from the traditional multi-class classification problem, this work focuses on discrete data space where the inputs $\x_{it},i\in[n],t\in[T_i]$, and the prediction embeddings corresponding to the labels $y_i,i\in[n]$ are all sampled from the same discrete set $\Eb$ with $K$ token embeddings. This setting can be directly applied to the language processing model where typically the dictionary size is fixed. 

To process the dataset $\data=(\X_i,y_i)_{i=1}^n$, We will create \emph{Next-Token Graphs} (NTG). An NTG is a directed graph with $K$ nodes (same as alphabet size). Dataset will be associated with multiple NTGs $(\Gck)_{k=1}^K$, each corresponding to a distinct value of the last token $\xl$. Concretely, $\Gck$'s are constructed as follows: 
\begin{enumerate}
    \item Split $\data$ into $K$ subsets $(\datak)_{k=1}^K$ with $\datak$ containing all input sequences that end with last token $\xl=\eb_k$.
    \item For any $(\X,y)\in\datak$, and for all $(y,x)$ pairs in $(\X,y)$ where $x$ is the correspinding token ID of $\x\in\X$, add a directed edge $(y\rightarrow x)$ into $\Gck$.
    % Consider all pairs $(y,\x)$ such that there is an input $(\Xs,y)$ in $\datak$ such that token index $x$ is in the sequence $\Xs$. For each $(y,x)$, add a directed edge $(y\rightarrow x)$ into $\Gck$.
\end{enumerate}
Note that nodes of $\Gck$ are subset of the indices $[K]$. The edges in $\Gck$ captures the priorities across tokens conditioned on the last token $\xl$. We will see that if there is a cycle (i.e., $(y\rightarrow x)$ and $(x\rightarrow y)$ are both in the graph), then, self-attention will assign comparable priorities to tokens $x,~y$. In contrast, if $y$ always \emph{dominates} $x$ (i.e.,~edges are always from $y$ to $x$), then, when $x,y$ are both present, self-attention will suppress $x$ and only select $y$ through the Attention-SVM mechanism observed in \cite{tarzanagh2023transformers}. \yl{[Lizzie: Need an intro figure, and add some discussion here.]}

To formalize this precisely, we need the notion of \emph{Strongly-Connected Components} (SCC). A directed graph is strongly connected if every node is reachable from every other node. SCCs of a directed graph form a partition into subgraphs that are themselves strongly connected. \yl{[Lizzie: add description based on the figure.]}

%For a graph $\Gc\in (\Gck)_{k=1}^K$, 
\red{\paragraph{SCCs and graph notation.} We can split a directed graph $\Gck$ into its SCCs, denoted as $(\Cck_i)_{i=1}^{N_k}$. Note that the number of SCCs in $\Gck$ denoted by $N_k$, is at most number of nodes. Hence in our case, it is upper bounded by $K$, and different SCCs within a same graph contain different nodes. Additionally, collapsing $\Cc_i$'s into individual nodes, we obtain the so-called \emph{condensation} $\Gcb$ of $\Gc$ which is a directed acyclic graph between SCCs. This condensation will essentially tell us the dominance order of SCCs.} We also introduce the following notation to denote node relations where $i,j\in[K]$ and $i\neq j$:%the order of nodes
\begin{itemize}
    \item $i\in \Gc$ denotes a node $i$ is inside $\Gc$.
    \item $(i\Rightarrow j)\in\Gc$ denotes a directed edge $(i\rightarrow j)$ is inside $\Gc$ but $(j\rightarrow i)$ is not.
    \item $(i \asymp j)\in\Gc$ denotes two nodes $(i,j)$ are in the same SCC of $\Gc$.
    %\item Given two SCCs $\Cc,\Cc'$, if $\Gcb$ contains a path from $\Cc$ to $\Cc'$, we use $\Cc\succ\Cc'$. 
    %\item If $i\in\Cc$ and $j\in\Cc'$ and $\Cc\succ\Cc'$, we denote $i\succ j$.
\end{itemize}


\red{\noindent \textbf{NTG of the dataset.} To recap, given $\data$, we construct its NTGs $(\Gck)_{k=1}^K$. For each $\Gck$, we obtain its SCCs denoted by $(\Cck_i)_{i=1}^{N_k}$ and condensation denoted by $\Gcbk$. The main contribution of this paper is establishing that NTGs capture the optimization geometry of the next-token prediction problem. Concretely, based on SCCs and condensation, we write the following Attention-SVM problem.}
\begin{align}\label{graph svm}\tag{Graph-SVM}
&\Wm=\arg\min_{\W}\tf{\W}\quad\\
&\text{s.t.}~~(\eb_i-\eb_j)^{\top}\W\eb_k
\begin{cases}=0\quad \forall(i\asymp j) \in\Gck\\
\geq 1\quad \forall(i\Rightarrow j)\in\Gck
\end{cases}
k\in[K].\nn
\end{align}
% \redp{Note that, in implementation, we only need to compare two SCCs once according to condensed graph $\Gcbk$. We don't need to worry about comparing all of their token pairs because equality constraints within SCCs will take care of it.}

When $(i\Rightarrow j)$, token ID $i$ has a higher \emph{priority} than $j$ and hence, SVM problem \eqref{graph svm} is finding the $\W$ such that $\W\eb_k$ achieves higher correlation to token embedding $\eb_i$ than $\eb_j$. While $(i\asymp j)$, there is not strict priorities between them, and hence we set the correlation difference equal to zero to prevent SVM solution $\W$ from distinguishing them.

{\color{red}
Finally, given $\data$, we define a subdataset induced by the interactions within SCCs. 
%\begin{definition}[Cyclic Subset]\label{cyc sub} $\cdata$ of $\data$ is obtained as follows. Pick a training example $(\Xs,y)\in \data$ iff it induces an edge in the SCC that contains $y$. That is, for some $x\in\Xs$ with $x\neq y$, $(x,y)$ are in the same SCC. Remove all tokens from $\Xs$ that are not in this SCC. Add $(\Xs,y)$ to $\cdata$.\end{definition}
\begin{definition}[Cyclic Subset]\label{cyc sub} $\cdata\subset\data$ is defined as follows. A training example $(\Xs,y)\in \data$ is an element of $\cdata$ if and only if it induces an edge in the SCC that contains $y$. That is, for some $x\in\Xs$ with $x\neq y$, $(x,y)$ are in the same SCC. Additionally, from $\cdata$, we obtain $\bdata$ by removing all tokens in $\Xs$ that are not in $y$'s SCC.\end{definition}

$\cdata$ and $\bdata$ are similar for all purposes but $\bdata$ provides a self-contained form that solely focuses on intra-SCC edges. Below we introduce acyclic dataset which will imply that next-token prediction has a strict priority order. This corresponds to the setting where all SCCs $\Cck_i$ are all singletons. It is also equivalent to $\cdata=\emptyset$.
}

Below we introduce acyclic dataset which will imply that next-token prediction has a strict priority order. 
\begin{definition}[Acyclic Dataset]\label{def acyc} We call $\data$ acyclic if all of its NTGs are directed acyclic graphs.
\end{definition}
For an acyclic dataset, we have no $i\asymp j\in\Gck$. Thus, the SVM formulation \eqref{graph svm} reduces to the following cleaner form.
\begin{align}\label{acyc svm}\tag{Acyc-SVM}
&\Wm=\arg\min_{\W}\tf{\W}\quad\\
&\text{s.t.}\quad (\eb_i-\eb_j)^\top\W\eb_k\geq 1\quad\forall(i\Rightarrow j)\in\Gck, ~k\in[K].\nn
\end{align}

\subsection{Technical Assumptions and the SVM Bias of Self-Attention}
In what follows, we will make a few assumptions that will make the optimization landscape of the problem more benign. Below, we discuss these and their justifications.

Since $\Cb$ choice is under our control and $\Eb$ is fixed, we choose $\Cb$ such that $k$'th row of $\Cb$ picks up token $k$ and suppresses other tokens. Concretely, we enforce the following criteria. 
%[$\cb_k$ picks up token $y$]
\begin{assumption}\label{assume iden} Classifier $\Cb$ and embeddings $\Eb$ satisfy $\Cb\Eb^\top=\Iden_K$.\todoasr{We can even share classifier and input embeddings, i.e., $\Cb = \Eb$. We will still need this assumption though.}
\end{assumption}
% \begin{assumption}[Relaxed]\label{assume relax} Suppose that for each row $k$, $\arg\max_{i\in[K]}\cb_k^\top\eb_i=k$.
% \end{assumption}
\redp{Later on, we can demonstrate that if this assumption is violated, global convergence of self-attention can in fact fail.}

\redp{If we call above Assumptions 1(a) and 1(b) it will appear more organized.}

Under Assumption \ref{assume iden}, the $k$'th entry of $\hat{\y}=\Cb\X^\top \sft{\X\W\xl}$ will return the likelihood of token $k$. The reason is that, $\sft{\X\W\xl}$ returns a probability distribution over tokens in the sequence and $\Cb\X^\top$ aggregates these probabilities into the token alphabet $[K]$. For instance, if a token $k$ shows up twice or more, $\Cb\X^\top$ will aggregate multiple occurrences into the $k$'th entry of $\hat{y}$. As a result, similar to cross-entropy loss, we assume that loss function only relies on $\hat{y}_y$ where $y$ is the true label.\todoasr{So we will not have an additional softmax operation on $\hat{\y}$ to convert it to a probability distribution?}
\begin{assumption}[Loss function]\label{assume loss} For any $\vb\in\R^K,y\in[K]$, we have $\ell(y,\vb)=\ell(\vb_y)$. Additionally, over the interval $[0,1]$, this scalar $\ell:\R\rightarrow\R$ is strictly decreasing, its derivative $\ell'$ is Lipschitz continuous, and $|\ell'|$ is bounded.
\end{assumption}

Under Assumption \ref{assume loss} above, we can write the ERM problem in a simplified form as follows
\[ 
\Lc(\Cb,\W)=\frac{1}{n}\sum_{i=1}^n \ell(\cb_{y_i}^\top\X_i^\top \sft{\X_i\W\xli}).
\]
Consider that $\Cb$ is fixed and we define two algorithms optimizing $\W$: 
\begin{itemize}
    \item Regularization path: Given $R>0$,
    \begin{align}\label{algo rp}\tag{Algo-RP}
    \bar\W_R=\arg\min_{\tf{\W}\leq R}\Lc(\W).
    \end{align}
    \item Gradient descent: Given starting point $\W(0)\in\R^{d\times d}$ and step size $\eta>0$, for $\tau\geq0$, 
    \begin{align}\label{algo gd}\tag{Algo-GD}
    \W(\tau+1)=\W(\tau)-\eta\nabla\Lc(\W(\tau)).
    \end{align}
\end{itemize}
\begin{lemma} \label{le:loss}
    Under Assumption \ref{assume loss}, $\nabla \Lc(\W)$ is $L$-Lipschitz continuous ,where $a_i = \|\cb_{y_i}\|\:\|\xli\|^2\|\X_i\|^3, b_i = M_0\|\cb_{y_i}\|\: \|\X_i\| + 3M_1$ for all $i \in [n]$
    \begin{equation} \label{eq:lwconst}
        L \coloneqq \frac{1}{n}\sum_{i=1}^n a_i b_i
    \end{equation}
\end{lemma}
We are now ready to state our first theorem on the global convergence of gradient descent. \redp{Note that assumptions ensure ``equal score'' guarantee of the other papers. The reason is that, score vector $\X_i\cb_{y_i}$ will be one-hot encoding i.e.~$1$ at the tokens $\eb_y$ and $0$ at the other tokens. Then, we can use Definition \ref{def acyc} so that solution is given by SVM form only (without a finite correction term).}
\begin{theorem}\label{thm:acyclic} Suppose $\data$ is acyclic per Definition \ref{def acyc} and Assumptions \ref{assume iden}\&\ref{assume loss} hold. Consider the GD iterations $\W_{k+1}=\W_k-\frac{1}{L}\nabla\Lc(\W_k)$ where $L$ is the smoothness of $\Lc(\W)$. Suppose \eqref{acyc svm} is feasible and $\Wm$ denotes its solution. Starting from any $\W_0$, we have that
\begin{align}
\lim_{k\rightarrow\infty}\frac{\W_k}{\tf{\W_k}}=\frac{\Wm}{\tf{\Wm}}
\end{align}
\redp{Additionally, under Assumptions \ref{assume iden}\&\ref{assume relax}, regularization path $W_R=\arg\max_{\tf{\W}\leq R}\Lc(\W)$ converges in direction to $\Wm$.}
\end{theorem}
\redp{I think \eqref{acyc svm} might be always feasible, especially if tokens are orthogonal or $K\leq d$. Please think about this.}

\redp{TODO: Above do we need the realizability assumption that next token is inside the sequence? See below.}

Recall that, 1-layer self-attention outputs a convex combination of the input tokens. If tokens are linearly independent, the only way model can output a target label $y$ would be if its embedding $\eb_y$ was inside the input sequence. This motivates the following realizability assumption.
\begin{assumption}[Realizable labels]\label{assume realizable} $\data$ is called realizable if for any $(\Xs,y)\in\data$, the label $y$ is contained in the sequence $\Xs$.
\end{assumption}
In fact, when token embeddings are orthonormal and $y$ is not realizable, the model can only make a random prediction over the output labels (since any output token is orthogonal to $\eb_y$). 

\redp{Additional Lemma: Under realizability, training error is zero whenever acyclic SVM is feasible.}

\redp{Potential Lemma (is this true?): Under realizability with $\ell(x)=-\log(x)$, the training loss is convex. If so, we could use this to establish global convergence of GD easier?}
% Additionally, it is strictly-convex over the cyclic subset \eqref{wfin soln}.

% \section{Main Results on Next-token Prediction}


==> sec/todo.tex <==
\section*{TODO?}
\begin{enumerate}
    \item Global and local discussion
    \item If realizability assumption, the attention weight $\W$ will potentially converge to the SVM solution but the graph is constructed via the selected tokens (or the token with higher scores in the sequence). 
    \item If $\Wm$ is not feasible, it might be related to the $\Wf$ but create SCC with finite tokens.
\end{enumerate}
